GazePrompt: Enhancing Low Vision People's Reading Experience with Gaze-Aware Augmentations

Reading is a challenging task for low vision people. While conventional low vision aids (e.g., magnification) offer certain support, they cannot fully address the difficulties faced by low vision users, such as locating the next line and distinguishing similar words. To fill this gap, we present GazePrompt, a gaze-aware reading aid that provides timely and targeted visual and audio augmentations based on users' gaze behaviors. GazePrompt includes two key features: (1) a Line-Switching support that highlights the line a reader intends to read; and (2) a Difficult-Word support that magnifies or reads aloud a word that the reader hesitates with. Through a study with 13 low vision participants who performed well-controlled reading-aloud tasks with and without GazePrompt, we found that GazePrompt significantly reduced participants' line switching time, reduced word recognition errors, and improved their subjective reading experiences. A follow-up silent-reading study showed that GazePrompt can enhance users' concentration and perceived comprehension of the reading contents. We further derive design considerations for future gaze-based low vision aids.

==> sections/old_6-study2.tex <==


\subsection{Study 2: Silent Reading Tasks}
\subsubsection{Participants}
We recruited 13 low vision participants (P4 - P16 in Table \ref{tab:lv_dem}), including ten female and three male whose ages ranged from 30 to 85 ($Mean = 58.62$, $SD = 19.62$). Among them, five participants were legally blind. No participants had other conditions that would cause reading difficulties other than their visual conditions. We recruited participants from a local low vision rehabilitation service. Before a potential participant was recruited, we conducted a screening interview via phone or email to check their eligibility. A participant was eligible if they were at least 18 years old and had low vision but still were able read with their residual vision. All participants completed the study without eye glasses. Participants were compensated \$20 per hour and were reimbursed for travel expenses. All participants completed the study except for P16 who only experienced the features and provided qualitative feedback due to an extensively long calibration process. 

\subsubsection{Procedure}
We conducted a single-session study in a well-lit environment. The study lasted 1.5 to 2 hours. The study included the following phases:

\textbf{\textit{Initial Interview \& Visual Acuity Test.}}
After obtaining participants' consent, we asked about their demographic information, visual condition, their challenges with daily reading, and their experience with assistive technology.  We then measured participants' visual acuity using letter-size ETDRS 1 and ETDRS 2 logMAR charts \cite{ferris1982new}. Participants were instructed to sit at four feet from the eye chart, and for those who could not see the largest row on the chart, we tested their visual acuity at 2 feet. They were asked to read chart 1 with their left eye covered, and then read chart 2 with the right eye covered. We recorded the smallest line that participants can recognize at least three out of five letters correctly. Our test covered a visual acuity range from 20/10 to 20/400. We used reported visual acuity for participants whose visual acuity was outside of the range (Table \ref{tab:lv_dem}).

\textbf{\textit{Gaze Calibration \& Validation.}} We then conducted gaze calibration with the participants, including both the 14-dot calibration and line-based correction, as described in Section \ref{sec:cal}. Participants sat in front of a computer screen with an eye tracker. After adjusting their position to achieve a horizontal distance of 65cm to the screen, participants were instructed to sit straight with their back touching the back of the chair to remain that position. We then adjusted screen height to align the participant's eye level with the center of the screen. Participants were asked to keep their body still in the study but small head movement was allowed when necessary. Before calibration, we adjusted the calibration target size for participants until they could locate the center of the target (the black dot) without eye squinting. They then completed the 14-dot calibration. A 5-dot validation followed, which collected the participants' calibrated gaze data when staring at five target and calculated the accuracy.  Finally, participants completed the line-based correction along with a 4-line validation, where we collected their corrected gaze data when tracking the moving target along four lines and calculated the accuracy. Based on the validation results, we decided which eye's data to use (left, right, or average) following the dominant-eye-based data collection \cite{wang2023understanding}, as well as whether or not to apply the line-based correction.

\textbf{\textit{Tutorial \& Customization.}} After calibration, we conducted a tutorial session to familiarize the participants with GazePrompt and allow them to customize the features. First, we showed participants an example passage and adjusted the font size, font weight, and color for participants so that they could read comfortably without eye squinting. We then introduced the LS and DW support in GazePrompt. For each feature, we demonstrated the two design alternatives and asked them to freely experience the feature on the example passage. During the exploration, participants customized the feature, including the augmentation color for the LS support, and the triggering time threshold for the DW support, until they were fully comfortable and familiar with it. We also asked for participants' feedback and suggestions on each design alternative. Participants also rated the effectiveness, comfort level, and distraction for each design alternative with a 7-point Likert scale score. Finally, we asked participants to select their preferred design alternative for each feature to use in the following reading tasks. 
%of this feature and how this feature works. We specifically mentioned that this feature achieves its best performance when the user conducts return sweep (also explained) for switching lines. 
%Next, we showed participants the two alternatives for this feature -- line highlighting and arrow, and had them adjust the color and brightness level to their preferred setting. 
%Participants then selected their preferred design alternative for each feature (line highlighting or arrow for LS support, and word magnifier or text-to-speech for DW support), and freely experienced the feature until they were fully familiar with it. We asked participants about the reasons behind their preference and customization. 
%Similarly, we introduced Difficult-Word Support to participants and showed them the two alternatives -- word magnifier and text-to-speech. They were asked to casually read an example passage with the default fixation duration thresholds, and asked about their opinions on the sensitivity of this feature. We increased the fixation thresholds if too many false positives were triggered, and reduced the fixation thresholds otherwise, until they were satisfied with the sensitivity level of the feature. 
%After the tutorial, we interviewed participants about their preference of the design of gaze-aware augmentations. 
 %they just experienced on a scale of 1 (strongly negative) to 7 (strongly positive), and corresponding rationales. We also prompted for suggestions to improve each feature. We let participants take a short break before proceeding to the next task.

\textbf{\textit{Reading Tasks.}} Participants performed multiple trials of reading tasks with and without GazePrompt. % we evaluated the effectiveness of GazePrompt through a series of reading tasks. Participant P16 did not proceed to this task due to time limit. %After the break, we had participants redo the calibration and validation process to ensure data quality. 
We adopted silent reading rather than reading aloud since it was more common in real world scenarios. 
%Then we introduced them the reading tasks. 
Participants read in four conditions: (1) without GazePrompt as the baseline, (2) LS support only, (3) DW support only, and (4) both LS and DW support. The passages were suitably magnified and adjusted to the participant's preferred contrast in all conditions to simulate the setup that they commonly used in daily reading. Participants were instructed to read as quickly as possible in the condition that they could build sufficient understanding of the passage. We asked two simple questions after each passage to ensure participants' basic comprehension on the reading content. 
We counterbalanced the four conditions using Latin Square \cite{bradley1958complete}. Six participants read two passages per condition, while the other six (P8, P9, P12-15) only read one passage per condition due to time constrain. We collected participants' gaze data in all reading tasks. 
%We collected their gaze data when reading passages. After participants finished reading four passages, we asked them to take a short break. After the break, six participants proceeded to recalibrate and read another four passages following the same procedure above, while the other six participants (P8, P9, P12-15) did not continue due to time limit or eye tiredness. Therefore, six participants read all eight passages and the others read four passages.

%four passages silently as quickly as possible, but they should have a basic understanding of the passage they read. After each passage, we had two simple questions for them to answer, which was only to verify that they had actually read the passage. Participants read each passage under one of the following conditions:

\textbf{\textit{Exit Interview.}} We ended our study with a semi-structured interview about participants’ reading experiences with GazePrompt. Participants rated the perceived accuracy, usefulness, and the learnability of GazePrompt on a scale of 1 (strongly negative) to 7 (strongly positive). We further asked about the use cases where GazePrompt could be useful, as well as their suggestions for improvements. %Then we asked about their experience with the combination of the two features. Lastly, we asked about their preference on gaze-controlled interaction versus traditional mouse/keyboard controlled interaction, and other features that can potentially support their reading inspired by GazePrompt. 

\subsubsection{Apparatus: Passage Preparation}
We selected reading passages from MCTest MC500 \cite{richardson2013mctest}, a dataset of passages with multiple-choice reading comprehension questions intended for machine comprehension. The passages were fictional stories, reducing the impact of participants' prior knowledge on passage comprehension. We selected 28 passages that were in similar length (about 177-199 words per passage) and at similar difficulty level (about 6th-grade level) according to the Flesch Reading Ease (FRE) score \cite{flesch1979write}. We manually checked each passage, ensuring no inappropriate contents were involved. Reading passages were randomly selected from this 28 passage dataset for each participant. 

%We first selected passages with a word count less than or equal to 200, and calculated the Flesch Reading Ease (FRE) score \cite{flesch1979write} for each passage. We selected the passages whose FRE scores are between 80 and 90 (about 6th-grade level). Lastly, two of our researchers went through the passages and removed those that were unreasonable or politically biased. The final set of passages used in our study contained 28 stories, each with two questions. The presentation of the passages was randomized for each participant. 

\subsection{Analysis}
Both quantitative and qualitative data were collected in the study. We first describe our quantitative analysis and then qualitative analysis.

%\subsubsection{Assessing Gaze Data Quality}
%\yuhang{start with the analysis goal... we first assessed the effectiveness of our calibration method with the line-based correction... }We had one within-in subject factor, \textit{CalibrationMethod} (\textit{WithLineCorrection}, \textit{WithoutLineCorrection}) and two measures: (1) \textbf{\textit{gaze recognition error in 5-dot validation}}, the mean visual angle difference between the target position and the estimated gaze location in the 5-dot validation, and (2) \textbf{\textit{gaze recognition error in 4-line validation}}, the mean vertical offset between the line position and estimated position of gaze points following each line. Neither of the measures was normally distributed based in Shapiro-Wilk test, so we used a repeated measure Aligned Rank Transform for Nonparametric Factorial ANOVA (ART) \cite{wobbrock2011aligned} to model the impact of line-based calibration on the two measures. 

\subsubsection{Effectiveness of LS support}
We first evaluated the effectiveness of the LS support. We defined three measures, including (1) \textbf{line switching time,} that is defined as the time between the last fixation at the end of the prior line and the first fixation that successfully lands on the next line followed by a forward saccade along that line. We calculated participants' mean line-switching time across all lines per passage.
%the gaze behavior from the moment the user finishes reading the current line, to the moment the user successfully finds the correct next line and start to perform the first forward saccade to read onward on that line. This measure describe the average time the user spent on line switching events.
(2) \textbf{frequency of line switching deviation}: we define a line switching deviation as an event when a user finishes reading the prior line and intends to switch to the next, their fixations accidentally land on a ``wrong'' line. We counted the total number of such events per passage as the deviation frequency. 
%The number of line switching events during which the user's gazes move to other lines.
(3) \textbf{magnitude of line switching deviation}, is defined as the distance between the wrong line and the target line in each deviation. We calculated the mean deviation magnitude per passage. 

%The average number of lines that are not the correct line where the user's gazes wander during a line switching deviation.
% \textbf{Line Switching Measures}: A line switching event is defined as the gaze behavior from the moment the user finishes reading the current line, to the moment the user successfully finds the correct next line and start to perform the first forward saccade to read onward on that line. We measure (a) the number of line switching events during which the user's gazes move to other lines, i.e., \textbf{number of lines with line switching errors}, and (b) the average number of lines that are not the correct line the user's gazes wander during a line switching error, i.e, \textbf{line switching error magnitude}.

% \textbf{Number of lines with line following errors}: A line following event is defined as the gaze behavior between two adjacent line switching events. This measure indicates the number of line following events during which the user's gazes move to other lines.

% \textbf{Line following error magnitude}: The average number of lines that the user's gazes cover during a line following error.

% \textbf{Line Following Measures}: A line following event is defined as the gaze behavior between two adjacent line switching events. Similarly, We measured (a) the number of line following events during which the user's gazes move to lines, i.e., \textbf{number of lines with line following errors}, and (b) the average number of lines that the user's gazes wander during a line following error, i.e, \textbf{line following error magnitude}.

We had one within-subject factor \textit{Condition}, including three levels: (1) without GazePrompt (\textit{Baseline}), (2) using LS support only, and (3) using both LS and DW support. %We compared the line switching measures and line following measures when participants read passages without GazePrompt, with Line-Switching/Following Support only, and with the combination of both features. 
To validate the counterbalancing, we involved another within-subject factor \textit{Order}, and found no significant effect of Order on any measures. We checked the normality of each measure using Shapiro-Wilk test. If a measure was normally distributed, we used ANOVA for analysis and Tukey's HSD for \textit{post-hoc} comparison if there was significance. Otherwise, we used ART and ART contrast test for \textit{post-hoc} comparison \cite{elkin2021aligned}. We used partial eta square ($\eta^2_p$) to calculate effect size for ART and ANOVA, with 0.01, 0.06, 0.14 representing the thresholds of small, medium and large effects, respectively \cite{cohen2013statistical}.


\subsubsection{Effectiveness of DW support}
We then evaluated the effectiveness of the DW support.
%can enable the user to more easily recognize an originally difficult words. 
We expect that the support would reduce the maximum time a user spends in recognizing a difficult word. We had one measure: \textbf{maximum one-pass fixation time on a word}---the maximum time a user fixates on a word within the first pass until their fixation switch to another word.

We had one within-subject factor \textit{Condition}, including three levels: (1) without GazePrompt (\textit{Baseline}), (2) using DW support only, and (3) using both LS and DW support. We also involved \textit{Order} as another within-subject factor and found no significant effect of Order on the measure, thus validating the counterbalance. Since not all participants had triggered the DW support (e.g., P4 has limited peripheral vision but relative good visual acuity), our analysis only focused on those who had the DW support triggered (7 participants). The statistical analysis process mirrors that in prior section. 

%removed participants who did not trigger any DW augmentation using the triggering time they were comfortable with. To validate the counterbalancing, we involved another within-subject factor \textit{Order}. \yuhang{validate the counterbalance here, no significant effect of order on measures.} We checked the normality of each measure using Shapiro-Wilk test. If a measure was normally distributed, we used ANOVA for analysis and Tukey's HSD for \textit{post-hoc} comparison if there was significance. Otherwise, we used ART and ART contrast test for \textit{post-hoc} comparison \cite{elkin2021aligned}. We used partial eta square ($\eta^2_p$) to calculate effect size for ART and ANOVA, with 0.01, 0.06, 0.14 representing the thresholds of small, medium and large effects, respectively \cite{cohen2013statistical}.

%\subsubsection{Exploratory Tests on Low Vision Conditions} During our study, we observed that different low vision conditions may affect users' performance with GazePrompt. We thus conducted post-hoc exploratory tests for unplanned comparisons, with Bonferroni correction \cite{armstrong2014use}. We defined two factors---\textit{VisualAcuity} and \textit{Visual Field}. \textit{VisualAcuity} had two levels, \textit{Low} and \textit{High}. Participants whose better eye visual acuity is better than 20/100 are considered as \textit{High}, otherwise, \textit{Low}. \textit{VisualField} had two levels: \textit{IntactPeripheralVision} and \textit{LimitedPeripheralVision} according to participants' self report. Similar to above analysis, for measures of interest that were normally distributed, we used ANOVA for analysis and Tukey's HSD for \textit{post-hoc} comparison if there was significance. Otherwise, we used ART and ART contrast test for \textit{post-hoc} comparison \cite{elkin2021aligned}.

\subsubsection{Qualitative Analysis} We video recorded the interviews and transcribed them using an online automatic transcription service. Our researchers then manually corrected the transcription errors. We analyzed the data using a standard qualitative analysis method \cite{saldana2021coding}. Two researchers independently coded three sample transcripts from three participants using open coding and generated a codebook upon agreement. Each researcher then coded half of the rest interviews based on the codebook, and updated the codebook upon agreement when new code emerged. Finally, we derived themes and categories based on the different aspects (e.g., effectiveness, user preferences) of the evaluated feature.

\subsection{Results}
\subsubsection{Gaze Data Quality} 
With our improved calibration procedure that involves line-based correction, the mean angular distance between the estimated gaze position and the target position in the 5-dot validation is 0.63\textdegree ($SD$ = 0.25\textdegree) viewed at 65cm from the screen, which is about 27 pixels on the screen. This result suggests that participants' gaze data were accurate enough for GazePrompt to function normally, since the smallest font size our participants chose was 48 pixels. Moreover, the percentage of data loss was 5.83\% ($SD$ = 7.50\%) which is much lower than the data loss (about 60\%) reported in prior work \cite{maus2020gaze}. Such high quality gaze data enabled GazePrompt to provide accurate gaze-aware augmentations. According to our participants, both Line-Switching Support and Difficult-Word Support were perceived to be highly accurate (LS: $Mean$ = 6.38 out of 7, $SD$ = 0.65; DW: $Mean$ = 6.54, $SD$ = 0.66). We report the effectiveness and participants' subjective feedback on the two features of GazePrompt below.

\subsubsection{Line-Switching Support} We report our quantitative and qualitative results about the performance of Line-Switching Support and participants' preference on the augmentation design.

\textbf{\textit{Line Switching Time (H1.1).}}
We found no significant effect of \textit{Condition}on line switching time \change{(ART: $F_{(2,22)} = 0.68$, $p = 0.516$, $\eta^2_p = 0.06$)}, \change{although the mean line switching time with GazePrompt ($Mean$ = 0.25s, $SD$ = 0.13s) was shorter than without ($Mean$ = 0.27s, $SD$ = 0.18s). We further looked into participants' gaze behavior during line switching events. We found that scrolling behavior was usually coupled with line switching behavior when participants finished reading the line at the bottom of the screen and ready to proceed to the next. Interestingly, participants tended to scroll longer distance in a single scrolling event (separated by 100 ms pause) (ANOVA: $F_{(2,22)} = 3.26$, $p = 0.06$, $\eta^2_p = 0.23$), resulting in significantly lower number of scrolling events (ART: $F_{(2,22)} = 5.43$, $p = 0.01$, $\eta^2_p = 0.33$). A post-hoc Tukey's HSD showed that Line-Switching Support significantly reduced the number of scrolling behavior by encouraging longer scrolling distance ($t_{(22)} = 3.23$, $p = 0.01$). This indicates that the ease of locating lines afforded by GazePrompt promoted longer scrolling distance, which in turn increased the time of line switching.}
% \yuhang{too negative... i'll report this together with the behavior change; so that it explained things a little}
% , although participants switched lines faster when using the combination of both feature ($Mean$ = 347.8 ms, $SD$ = 122.3 ms) than without GazePrompt ($Mean$ = 362.1 ms, $SD$ = 141.0 ms). 

\textbf{\textit{Number of Line Switching Deviation (H1.2).}}
Participants had significantly less line switching deviations \change{(ART: $F_{(2,22)} = 8.00$, $p = 0.002$, $\eta^2_p = 0.42$)} when using GazePrompt than without GazePrompt. A \textit{post-hoc} ART contrast test showed that the participants had less line switching deviations when using Line-Switching Support than without GazePrompt \change{($t_{(22)} = 4.00$, $p = 0.002$)}. 
% Interestingly, Participants had more line switching deviations when using Line-Switching Support only than the combination of both features ($t_{(22)} = -2.65$, $p = 0.04$). Our H1.2 was verified. This result also indicates that with full GazePrompt support, participants could switch lines smoother than Line-Switching Support only. Some participants did mention relying on the Difficult-Word Support to help locate lines, as P12 mentioned, \textit{``If I'm at the end of the sentence... If it reads to me, and like, let's say if there's a sentence that says, `The dog chased the ball,' then there'll be on the word `ball,' and then I know, okay, that's the end of the sentence. Now, I know that I'll have to read another sentence...''}

\textbf{\textit{Line Switching Deviation Magnitude (H1.3).}}
We found \textit{Condition} had significant effect on line switching deviation magnitude \change{(ART: $F_{(2,22)} = 3.98$, $p = 0.03$, $\eta^2_p = 0.27$)}. A \textit{post-hoc} ART contrast test showed that the participants' gaze deviated to less lines during line switching events when using the combination of both features than without GazePrompt \change{($t_{(22)} = 3.74$, $p = 0.003$)}, however, no significant difference was found between Line-Switching Support only and without GazePrompt ($t_{(22)} = 1.43$, $p = 0.34$). Our H1.3 was partially verified since Line-Switching alone did not effectively reduce line switching deviation magnitude. \yuhang{this sounds like the DW feature helps with the line deviation magnitude... which does not make much sense.}

% As for line following measures, there was on significant effect of \textit{Condition} on the number of line following deviations (ART: $F_{(2,22)} = 0.67$, $p = 0.52$, $\eta^2_p = 0.06$), however, \textit{Condition} had significant effect on line following deviation magnitude. Participants' gazes deviated to significantly more line when following a line using the combination of both features than Line-Switching/Following Support only ($t_{(23)} = -2.71$, $p = 0.03$). There was no significant difference on line following deviation magnitude between no support and Line-Switching/Following Support only ($t_{(23)} = 0.49$, $p = 0.88$), and between no support and the combination ($t_{(23)} = -2.22$, $p = 0.08$).

\begin{figure*}[h]
  \includegraphics[width=0.95\textwidth]{sections/pics/fig4-scroll.png}
  \caption{GazePrompt changed participants' scrolling behavior. Orange dots represent fixations and blue and red line segments represent forward and backward saccades, respectively. (a) P6 scrolled two lines up from bottom while her fixation went up to track the line starting with ‘thing’ that she was reading when not using LS Support; (b) P6 scrolled six lines up from bottom while her fixation went up to track the line starting with ‘helping’ that she was reading when using LS Support}
  \label{fig:scroll}
    \vspace{-2ex}
\end{figure*}

% \textbf{\textit{Scrolling behavior change.}} Since the increased font size required participants to scroll up and down using the scroll wheel on the mouse, We further looked into their scrolling behavior change caused by GazePrompt. We found that participants on average scrolled longer distance (i.e., scrolling magnitude) in a single scrolling event (separated by 100 ms pause) when using GazePrompt (ANOVA: $F_{(2,22)} = 3.98$, $p = 0.03$, $\eta^2_p = 0.27$). A post-hoc Tukey's HSD showed that participants had significantly lower scrolling magnitude reading without GazePrompt than using Line-Switching Support only ($t_{(22)} = -3.23$, $p = 0.01$). This indicated that GazePrompt could potentially change participants' scrolling behavior, and participants could scroll longer distance each time to reveal the hidden text because Line-Switching Support made locating lines easier. Figure \ref{fig:scroll} shows an example where P6 scroll the current line to the top directly with GazePrompt, versus she only scrolled two lines up at a time without GazePrompt.

\begin{figure*}[h]
  \includegraphics[width=\textwidth]{sections/pics/fig5-likert@2x.png}
  \caption{The distribution of participants' answers to 7-point Likert scale questions about the two features of GazePrompt.}
  \label{fig:likert}
    \vspace{-2ex}
\end{figure*}

\begin{figure*}[h]
  \includegraphics[width=0.95\textwidth]{sections/pics/fig-pref.png}
  \caption{Participants' preference on the two features of GazePrompt. The first column shows participants' preference on Line-Switching Support design along with their text setting. Magnifier icon represents word magnifier, and speaker icon represents Text-to-Speech.}
  \label{fig:pref}
    \vspace{-2ex}
\end{figure*}

\textbf{\textit{Preference on Different Augmentation Design.}} Out of 13 participants, 11 preferred line highlighting. Figure \ref{fig:likert} presents participants' scores for likert-scale questions. Participants felt the line highlighting was effective ($Mean$ = 6.53, $SD$ = 0.66). All participants agreed that line highlighting improved their focus on the line they are reading. 4 participants believed the highlighting provided enough contrast for participants to stay focused on what they are reading. Some participants mentioned the line highlighting made text more "digestible" because the line they read was separated from other part of the text. As P5 mentioned, \textit{``I like having it (line highlighting) distinguish exactly what I'm supposed to be staring at... For me. If it's in a big format like this [passage], sometimes it's easier if it's broken into smaller chunks [by the highlighting].``} Participants found line highlighting comfortable to see ($Mean$ = 6.62, $SD$ = 0.65). P9 explicitly explained that line highlighting reduced her eye strain when reading compared to reading without it, thus improved her reading experience, \textit{``If you're straining to see something... You're focusing on the straining. Not on what you are reading.``} Although participants in general felt that line highlighting was not distracting ($Mean$ = 2.31, $SD$ = 1.55), participants' opinions differed. Seven participants enjoyed using line highlighting since it was not distracting at all. Moreover, line highlighting could even make reading less distracting for participants with peripheral vision loss. For example, P4 described her peripheral vision as flashing static noise on old TVs, which can be distracting during reading. With line highlighting, she could focus on the text better, \textit{``Sometimes like especially when I'm trying to focus on a word that (peripheral vision) will be like the static [noise]... more distracting, whereas the highlighting made it go away because I was focused on the color and the highlighting and the words.``} Participants who thought line lighting was distracting because of the sudden change of text background color caused by line highlighting when participants switched lines (P7, P13). P7 complained that it took her one second or two to get used to the highlighting on the next line after a line switching.  

Although the arrow was less popular among our participants with lower effectiveness ($Mean$ = 4.54, $SD$ = 1.76), lower comfort level ($Mean$ = 5.69, $SD$ = 1.38) and slightly higher distractiveness ($Mean$ = 3.15, $SD$ = 2.41), two participants still preferred the arrow to the line highlighting for their LS support. Participants who liked the arrow said it improved focus (P4) and was less distracting than line highlighting, because it was easier to ignore when they did not need it during reading (P7, P11). However, this advantage of the arrow was also the reason why other participants disliked the arrow. Since the arrow was placed at the beginning of each line, it was more difficult for people with peripheral vision loss to spot than the line highlighting (seven participants). Such issue led participants to spend extra time searching for the arrow, which slowed down reading (P5, P8, P9, P12) and caused eye strain (P7, P16). Beside, seven participants disliked the fact that the arrow only supported locating the beginning of the line instead of following the line, like P5 mentioned, \textit{``It's just that the arrow points at which line I'm on, whereas the line highlighting tells me exactly what words I'm reading.``} Furthermore, participants' attention was stolen from the text by the arrow (five participants). P14 explained that having to focus on the arrow interrupted her flow of reading, \textit{``This one (arrow), I have to keep focusing on the little triangle on the left. So it forces you to spend more time looking at that triangle or having your focus on it.``}. Lastly, some participant (P7) felt the position of the arrow was too close to the first word on the line, which might hinder their ability to recognize the word.

Participants liked the fact that they could change the color of the augmentations (P13, P14). Figure \ref{fig:pref} presents participants' choices of augmentation design and color. All participants chose the color that created high contrast to the text. Four participants made the color dimmer to further increase the contrast between the text and highlighting. However, participants did not need enough contrast between the highlighting color and background color to be able to distinguish the highlighted line from others. \yuhang{what does this mean? if they cannot distinguish the line from others, how the feature is helpful?}

\textbf{\textit{Subjective Feedback on System Performance.}} Participants' feedback on the performance of Line-Switching/Following Support was very positive. They overall felt this feature was useful ($Mean$ = 6.50, $SD$ = 0.80). The major concern about this feature would be the speed when the change of augmented line was triggered. While five participants liked the responsiveness of the line changing mechanism, P4 and P11 said the change of the augmented line was too fast, and three participants felt there was a little delay on when the feature changes augmented lines. Besides, two participants reported the features jumped lines by itself when they were not changing lines. These issues might be because participants' estimated fixations spilled over to other lines for a relatively long time which triggered the line change. \yuhang{not interesting... sounds like technical report, but essentially, it's just the eye tracking is not that accurate; consider remove.}

\textbf{\textit{Suitable Use Cases \& Potential Improvement}}
Participants brainstormed the use cases Line-Switching Support can be most helpful, and potential improvement of this feature to help improve their reading experience. Four participants believed this feature could be particularly helpful when reading long and technical passages that require a certain level of concentration. P7 said Line-Switching Support can be more helpful when reading text with smaller line spacing. Due to the inconvenience of the position of the arrow, three participants suggested placing the arrow on both sides of the screen, which could be more useful for participants with peripheral vision loss who could not perceive the left side of the screen as effectively. Due to severe peripheral vision loss (tunnel vision), P16 further suggested making the arrow blink to help him locate the line faster. Inspired by line highlighting, P4 and P10 suggested a word-level highlighting which could provide even more targeted support on individual words on a line. Besides highlighting, P4 thought underlining can be a more ideal option that is less obtrusive than highlighting, but more salient than arrow as the user read along a line. Finally, P9 commented on color options of GazePrompt, and suggested automatic color setting based on the lighting condition in the room and the brightness of the screen.

\subsubsection{Difficult-Word Support} We report our quantitative and qualitative results about the performance of Difficult-Word Support and participants' preference on the augmentation design.

\textbf{\textit{Maximum one-pass per-word fixation time (H2).}} Using a repeated-measure ANOVA, we did not find significant effect of \textit{Condition} on the maximum time participants fixated on a word \change{($F_{(2,11)} = 1.85$, $p = 0.20$, $\eta^2_p = 0.25$)}, although the mean value shows that participants using LS+DW had smaller maximum one-pass per-word fixation time \change{($Mean$ = 1942.8 ms, $SD$ = 835.2 ms)} than DW only \change{($Mean$ = 2038.5 ms, $SD$ = 796.4 ms)}, and without GazePrompt \change{($Mean$ = 2260.3 ms, $SD$ = 947.0 ms)}. \change{While Difficult-Word Support was supposed to be used when recognizing certain words by vision was difficult, four participants mentioned using it as a confirmation to the words they could recognize by vision but not confident about. As P5 commented, \textit{``when it (Text-to-Speech) would say it, my brain went `Yes! Yes! That is the word I just saw.'''} She further explained her preference on reading accuracy over speed, \textit{``(reading) Speed... I gave up on that a long time ago... Because if I go into my own world (not for the purpose of the study), I don't focus on speed at all. I like accuracy, not speed. Speed is for fast food.''} P4 even intentionally chose longer fixation duration thresholds to use their gaze as command versus an assistance responding to their natural reading behavior. As such, Difficult-Word Support might have also been used as a double-check tool in pursuit of reading accuracy and high confidence, therefore, overshadowing its ability to reduce word recognition time.}
% This result contradicted our hypothesis H2. The Difficult-Word support might be able to help participants recognize the word that are difficult to read, but that does not necessarily transfer to faster word recognition speed. \yuhang{the comments are too arbitrary...sounds quite negative. rewrite.}
% Further experiments need to be conducted to evaluate the potential of Difficult-Word support in facilitating reading accuracy.
% as P2 pointed out, \textit{``Because (reading) speed... I gave up on that a long time ago... Because if I go into my own world (not for the purpose of the study), I don't focus on speed at all. I like accuracy, not speed. Speed is for fast food.

\textbf{\textit{Preference on Different Augmentation Design.}} 
11 Participants chose Text-to-Speech to be their DW support (Fig. \ref{fig:pref}). \yuhang{need a paragraph, or a section to discuss the parameter preferences, and what we learn from it. anything in common across participants for the fixation time to define difficulty word? } Participants liked this augmentation because it accurately detected difficult words and made them easier to recognize, as P5 commented, \textit{``It definitely was reading all of the words that I either scanned more than once or took more than a second... because my eyeballs have to focus on each word almost individually.``}. Participants agreed that Text-to-Speech was comfortable to use ($Mean$ = 6.23, $SD$ = 1.24), because it reduces eye strain while being able to react to the user's gaze (P5, P12). 
% because they did not need to divert their gaze to somewhere else to locate the word which reduced their eye strain (P5, P11, P12). 
Participants did not think Text-to-Speech was distracting ($Mean$ = 2.08, $SD$ = 1.44). Some participants (P4, P12) liked the fact that it was easier to ignore when not needed which is better than not having it, as P12 mentioned, \textit{``I'm not distracted by text-to-speech. It doesn't affect me when I'm reading like, I would rather that than not have it.``} In addition to the high saliency and low distractiveness, three participants acknowledged that this augmentation recognized difficult words faster than themselves, which made some participants felt they read slow with their eyes, as P5 explained, \textit{``I read slow. And this thing (Text-to-Speech) makes it very obvious that I read slow. Because it picks up words quicker than I do.``} 
% Furthermore, four participants liked Text-to-Speech because it helped users to examine whether they read the correct word or not. P13 had central vision loss which causes some letters in a word disappear, and she felt Text-to-Speech was particularly helpful for people like her, \textit{``For those who miss letters in a word... that can be clarified with [Text-to-] speech.``}
Despite the responsiveness afforded by Text-to-Speech, it has several drawbacks. Five participants reported the speech interrupted their mental process, and even made them forgot what they read, as P14 complained, \textit{``I ended up losing my spot sometimes. Because my brain is listening to the word. And now I'm trying to find where I was.``}
Moreover, participants (P6, P7, P9, P10) found the audio modality to be obtrusive, and the startling sound made them feel uncomfortable. 

Word magnifier was considered less effective ($Mean$ = 4.77, $SD$ = 2.13), less comfortable ($Mean$ = 5.08, $SD$ = 2.25) and more distracting ($Mean$ = 4.46, $SD$ = 2.44) compared to Text-to-Speech. Participants complained about the visual design of word magnifier. To start with, there was not enough padding space between the magnified text and the border of the magnifier, making it difficult to recognize the first letter of word (P11); Participants with peripheral vision loss could not see the full magnified word without moving their eyes to search for it. Four participants mentioned the magnifying factor was larger than necessary which caused distraction to reading. Besides the visual design, the disappearance of the magnifier when the user moves their eyes away caused a sense of lost and even more distraction (P5, P7, P11). For example, P11 found it difficult to navigate back to where he left off when the magnifier disappeared, \textit{``When it magnified [the word,] it blocked the rest of the words. And so it was hard to get my track back when it disappeared. I wasn't sure 'was it here? Or was it here?' So it was hard to restart (resume) reading afterwards.``} Even with improved design for word magnifier, P11 conveyed their doubt about whether word magnifier was a good design, since for some low vision users, the word recognition issue could not be addressed by magnification.
Participants who liked word magnifier said it made the difficult word distinct from other words (P4, P8-P10), which improved reading comprehension and speed for low vision people who prefer visual input than auditory, as P4 said, \textit{``I like the magnifier because I think it is the way I learn better, and [it] pulls the word out and is less distracting than having it said... I'm not as auditory of a learner.`}

\textbf{\textit{Subjective Feedback on System Performance.}} No matter which augmentation participants chose, they agreed that Difficult-Word Support was useful ($Mean$ = 5.83, $SD$ = 1.59). Nine out of 13 participants would like to use this feature regularly because of the ease of recognizing difficult words with it. The major complaint of Difficult-Word Support was on the sensitivity level. Although all participants adjusted the fixation duration to fit their reading and eye using habits, two participants felt there was a delay before the difficult word was triggered, whereas five participants felt it was too sensitive for simple words (e.g., a, the, to) they did not need assistance with. P5 further mentioned the over-sensitivity attracted her attention, which in turn slowed down her reading. Despite the effectiveness of Difficult-Word Support acknowledged by most participants, further experiment is needed to optimize the difficult word detection strategy to better suit participants' own needs. \yuhang{the sensitivity sounds to be a parameter adjustment issues...which is not interesting.}

\textbf{\textit{Suitable Use Cases \& Potential Improvement}}
Seven participants proposed that Difficult-Word Support would be most helpful in unfamiliar word recognition, such as names (P7) and terminologies in textbooks (P6). Two participants said it was helpful for important and long words. Participants brought up different ideas on improving the current Difficult-Word Support. Two participants suggested color options for the magnified text and its background to make the word stand out even more among all the words. One participants would like the magnifier to be displayed on the same line as the original word to prevent losing context when reading. Finally, the system default voice for Text-to-Speech was considered unnatural by P10 and P14, so a customizable voice would be desired.

\subsubsection{Overall Reading Experience with GazePrompt}
% as P2 pointed out, \textit{``Because (reading) speed... I gave up on that a long time ago... Because if I go into my own world (not for the purpose of the study), I don't focus on speed at all. I like accuracy, not speed. Speed is for fast food.``} 
% By instructing participants to read silently as quickly as possible, we aimed to simulate a natural reading scenario. Participants expressed different opinions on how their daily reading was like. P5 explained the reason she prioritize reading accuracy to speed, \textit{``I gave up on that a long time ago... Because if I go into my own world (not for the purpose of the study), I don't focus on speed at all. I like accuracy, not speed. Speed is for fast food.``}
Participants all had positive experiences with GazePrompt. Although they all agreed both features provided by GazePrompt were easy to learn (LS: $Mean$ = 6.92, $SD$ = 0.29; DW: $Mean$ = 6.83, $SD$ = 0.58), eight participants said they would be more comfortable using GazePrompt by practicing more. Seven participants like the combination more than individual features because it could provide assistance to improve reading experience in different aspects, as P4 explained, \textit{``But then when I was stuck on a word and the highlighting wasn't helping and the magnification of it made it quite clear. So then I could focus on just the individual word. So I think overall the experience was heightened and way more positive with both of them together.``} 

When asked about their experience with gaze-aware augmentations, nine participants preferred gaze-control than traditional mouse and keyboard control, because gaze-control was faster (P6-P9, P11, P14) and more natural (P10, P13). Because using their vision to find the keyboard or mouse itself added to their visual burden. For example, P7 mentioned, \textit{``[With gaze-control] I can just look at the word and it will recognize that I'm looking at it, instead of trying to locate my cursor on the screen and then move it to that word.``} P16 usually used screen reader for his daily tasks. Despite his limited visual field, he preferred the Text-to-Speech feature to conventional keyboard/mouse controlled screen reader, since it provided targeted support and did not read everything on the screen.
However, participants (P5, P7, P12) who preferred traditional input method expressed their concern about their ability to control their gaze. With certain visual conditions, controlling their eye movement can be difficult. Using their eyes to interact with the system can cause dry eyes and eye strain, as P12 commented, \textit{``I like the mouse and keyboard control better. Because I'm able to physically control where I'm at. Instead of having, like [gaze control], it's (mouse and keyboard control) less strain on my eyes.``}.
Future research should provide both gaze input and conventional input modality for low vision users to choose.

